DYSAN: Dynamically sanitizing motion sensor data against sensitive inferences through adversarial networks

With the widespread adoption of the quantified self movement, an increasing number of users rely on mobile applications to monitor their physical activity through their smartphones. Granting to applications a direct access to sensor data expose users to privacy risks. Indeed, usually these motion sensor data are transmitted to analytics applications hosted on the cloud leveraging machine learning models to provide feedback on their health to users. However, nothing prevents the service provider to infer private and sensitive information about a user such as health or demographic attributes.In this paper, we present DySan, a privacy-preserving framework to sanitize motion sensor data against unwanted sensitive inferences (i.e., improving privacy) while limiting the loss of accuracy on the physical activity monitoring (i.e., maintaining data utility). To ensure a good trade-off between utility and privacy, DySan leverages on the framework of Generative Adversarial Network (GAN) to sanitize the sensor data. More precisely, by learning in a competitive manner several networks, DySan is able to build models that sanitize motion data against inferences on a specified sensitive attribute (e.g., gender) while maintaining a high accuracy on activity recognition. In addition, DySan dynamically selects the sanitizing model which maximize the privacy according to the incoming data. Experiments conducted on real datasets demonstrate that DySan can drasticallylimit the gender inference to 47% while only reducing the accuracy of activity recognition by 3%.

==> bib_ecml.tex <==
\begin{thebibliography}{}

\bibitem{7962470}
A.Abadleh, E.Al-Hawari, E.Alkafaween and H.Al-Sawalqah,
Step detection algorithm for accurate distance estimation using dynamic step length,
MDM,
324-327,
(2017)

\bibitem{aivodji2019agnostic}
  U.Aivodji, F.Bidet, S.Gambs, R.C.Ngueveu and A.Tapp,
  Agnostic data debiasing through a local sanitizer learnt from an adversarial network approach,
  ArXiv arXiv:1906.07858,
  (2019)


\bibitem{alzantot2017sensegen}
  M.Alzantot, S.Chakraborty, and M.Srivastava,
  Sensegen: A deep learning architecture for synthetic sensor data generation,
  PerCom Workshops,
  188--193,
  (2017)

\bibitem{steps}
C.BenAbdelkader, R.Cutler and L.Davis,
Stride and cadence as a biometric in automatic person identification and verification,
FGR,
372-377,
(2002)


\bibitem{dtw}
 D.J.Berndt and J.Clifford,
 Using Dynamic Time Warping to Find Patterns in Time Series,
 AAAIWS,
 359-370,
 12,
 (1994)

\bibitem{chakraborty}
 S.Chakraborty, K.R.Raghavan, M.P.Johnson and M.B.Srivastava,
 A Framework for Context-Aware Privacy of Sensor Data on Mobile Systems,
HotMobile,
6,
 (2013)

\bibitem{chen2018vganbased}
    C.Jiawei, K.Janusz and I.Prakash,
    VGAN-Based Image Representation Learning for Privacy-Preserving Facial Expression Recognition,
    ArXiv arXiv:1803.07100,
    (2018)


\bibitem{edwards2015censoring}
    E.Harrison and S.Amos,
    Censoring Representations with an Adversary,
    ArXiv arXiv:1511.05897,
    (2015)

\bibitem{DLReview}
   H.Ismail Fawaz, G.Forestier, J.Weber, L.Idoumghar and P.Muller,
   Deep learning for time series classification: a review,
   Data Mining and Knowledge Discovery,
   33,
   4,
   917-963,
   (2019)

\bibitem{Feldman2014}
  M.Feldman, S.A.Friedler, J.Moeller, C.Scheideggera and S.Venkatasubramanian,
  Certifying and removing disparate impact,
  KDD,
  259--268,
  (2015)

\bibitem{stroke1}
 G.D.Fulk and E.Sazonov,
 Using Sensors to Measure Activity in People with Stroke,
 Topics in Stroke Rehabilitation,
 18,
 6,
 746-757,
  (2011)

\bibitem{han2012accomplice}
  J.Han, E.Owusu, L.T.Nguyen, A.Perrig and J.Zhang,
  Accomplice: Location inference using accelerometers on smartphones,
  COMSNETS,
  1--9,
  (2012)

\bibitem{jourdan2018toward}
  T.Jourdan, A.Boutet and A.Frindel,
  Toward privacy in IoT mobile devices for activity recognition,
  MobiQuitous,
  155--165,
  (2018)


\bibitem{kroger2019privacy}
  J.L.Kr\"oger, P.Raschke and T.R.Bhuiyan,
  Privacy implications of accelerometer data: a review of possible inferences,
  ICCSP,
  81--87,
  (2019)


\bibitem{lee2002activity}
  S.Lee and K.Mase,
  Activity and location recognition using wearable sensors,
  Pervasive Computing,
  1,
  3,
  24--32,
  (2002)


\bibitem{liu2017deeprotect}
    C.Liu, S.Chakraborty and P.Mittal,
    DEEProtect: Enabling Inference-based Access Control on Mobile Sensing Applications,
    ArXiv arXiv:1702.06159,
    (2017)


\bibitem{Malekzadeh2018}
  M.Malekzadeh, R.G.Clegg, A.Cavallaro and H.Haddadi,
  Protecting Sensory Data Against Sensitive Inferences,
  W-P2DS,
  2:1--2:6,
  6,
  (2018)
 
\bibitem{Malekzadeh_2019}
   M.Malekzadeh, R.G.Clegg, A.Cavallaro and H.Haddadi,
   Mobile sensor data anonymization,
   IoTDI,
   (2019)


\bibitem{menasria}
  S.Menasria, J.Wang and M.Lu,
  The purpose driven privacy preservation for accelerometer-based activity recognition,
  WWW,
  21,
  1773-1785,
  (2018)

\bibitem{demontjoye2013unique}
   Y.de Montjoye, C.A.Hidalgo, M.Verleysen and V.Blondel,
   Unique in the Crowd: The privacy bounds of human mobility,
   Nature,
    3,
    (2013)


\bibitem{nweke2018deep}
  H.F.Nweke, Y.W.Teh, M.A.Al-Garadi and Alo, R.Uzoma,
  Deep learning algorithms for human activity recognition using mobile and wearable sensor networks: State of the art and research challenges,
  Expert Systems with Applications,
  105,
  233--261,
  (2018)

\bibitem{oleszkiewicz2018siamese}
    W.Oleszkiewicz, P.Kairouz, K.Piczak, R.Rajagopal and T.Trzcinski,
    Siamese Generative Adversarial Privatizer for Biometric Data,
    ArXiv arXiv:1804.08757,
    (2018)


\bibitem{pan2019recent}
  Z.Pan, W.Yu, X.Yi, A.Khan, F.Yuan and Y.Zheng,
  Recent progress on generative adversarial networks (GANs): A survey,
  Access,
  7,
  36322--36333,
  (2019)

\bibitem{stroke2}
H.Park, H.Chang and H.S.Nam,
Use of Machine Learning Classifiers and Sensor Data to Detect Neurological Deficit in Stroke Patients,
J Med Internet Res,
19,
4,
e120,
(2017)



\bibitem{park2018data}
  N.Park, M.Mohammadi, K.Gorde, S.Jajodia, H.Park and Y.Kim,
  Data synthesis based on generative adversarial networks,
  VLDB,
  11,
  10,
  1071--1083,
  (2018)

\bibitem{qi2015survey}
  J.Qi, P.Yang, D.Fan and Z.Deng,
  A survey of physical activity monitoring and assessment using internet of things technology,
  CIT/IUCC/DASC/PICOM,
  2353--2358,
  (2015)


  
\bibitem{ramasamy2018recent}
  S.R.Ramamurthy and N.Roy,
  Recent trends in machine learning for human activity recognition-A survey,
  Wiley Interdisciplinary Reviews: Data Mining and Knowledge Discovery,
  8,
  4,
  (2018)

\bibitem{olympus_raval}
        N.Raval, A.Machanavajjhala and J.Pan,
        Olympus: Sensor Privacy through Utility Aware Obfuscation,
        PETS,
        5 - 25,
        1,
        (2019)


\bibitem{ortiz2015smartphone}
	J. L.Reyes-Ortiz,
	Smartphone-based human activity recognition,
	Springer,
	(2015)


\bibitem{DBLP:s/corr/abs-1904-01059}
M.Romanelli, C.Palamidessi, K.Chatzikokolakis, Generating Optimal Privacy-Protection Mechanisms via Machine Learning, CoRR, abs/1904.01059, (2019)


\bibitem{schafer2019competitive}
  F.Sch\"afer and A.Anandkumar,
  Competitive gradient descent,
  NIPS,
  7623--7633,
  (2019)


\bibitem{sprager2015inertial}
  S.Sprager and M. B.Juric,
  Inertial sensor-based gait recognition: a review,
  Sensors,
  15,
  9,
  22089--22127,
  (2015)


\bibitem{tedesco2017review}
  S.Tedesco, J.Barton and B.O'Flynn,
  A review of activity trackers for senior citizens: Research perspectives, commercial landscape and the role of the insurance industry,
  Sensors,
  17,
  6,
  1277,
  (2017)


\bibitem{tripathy2019privacy}
  A.Tripathy, Y.Wang and P.Ishwar,
  Privacy-preserving adversarial networks,
  Allerton,
  495--505,
  (2019)


\bibitem{vavoulas2016mobiact}
  G.Vavoulas, C.Chatzaki, T.Malliotakis, M.Pediaditis and M.Tsiknakis,
  The MobiAct Dataset: Recognition of Activities of Daily Living using Smartphones.,
  ICT4AgeingWell,
  143--151,
  (2016)



\bibitem{yang2016user}
  H.Yang J.Yu, H.Zo and M.Choi,
  User acceptance of wearable devices: An extended perspective of perceived value,
  Telematics and Informatics,
  33,
  2,
  256--269,
  (2016)


\bibitem{zarepour}
  E.Zarepour, M.Hosseini, S.S.Kanhere and A.Sowmya,
  A context-based privacy preserving framework for wearable visual lifeloggers,
  PerCom, 
  1-4,
  (2016)
  
\end{thebibliography}{}


==> comment.tex <==

\definecolor{mygray}{gray}{0.2}
\definecolor{mycyan}{rgb}{0.05, 0.5, 0.5}

\def\red#1{\textcolor{red}{#1}}
\def\blue#1{\textcolor{blue}{#1}}
\def\green#1{\textcolor{green}{#1}}
\def\magenta#1{\textcolor{magenta}{#1}}
\def\orange#1{\textcolor{orange}{#1}}
\def\darkcyan#1{\textcolor{mycyan}{#1}}
\def\gray#1{\textcolor{mygray}{#1}}


\def\remark#1#2#3{        
% 1 = name; 2 = color; 3 = comment
  \ifediting
        \todo[color=#2]{#1: #3}
    \fi
    }

\def\newtext#1#2#3{        
% 1 =  name; 2 = color; 3 = text
  \ifediting
        %\textcolor{#2}{\textbf{#1 wrote: }\\ #3}
        \textcolor{#2}{\textbf{#1: } #3}
    \else 
        {#3}
    \fi
    }
    
\def\AB#1{\remark{Antoine}{cyan!30}{#1}}
\def\CF#1{\remark{Carole}{magenta!30}{#1}}
\def\TJ#1{\remark{Theo}{teal!30}{#1}}
\def\SG#1{\remark{Sebastien}{orange!30}{#1}}
\def\RN#1{\remark{Rosin}{violet!30}{#1}}


